A Scalable Space-efficient In-database Interpretability Framework for Embedding-based Semantic SQL Queries

AI-Powered database (AI-DB) is a novel relational database system that uses a self-supervised neural network, database embedding, to enable semantic SQL queries on relational tables. In this paper, we describe an architecture and implementation of in-database interpretability infrastructure designed to provide simple, transparent, and relatable insights into ranked results of semantic SQL queries supported by AI-DB. We introduce a new co-occurrence based interpretability approach to capture relationships between relational entities and describe a space-efficient probabilistic Sketch implementation to store and process co-occurrence counts. Our approach provides both query-agnostic (global) and query-specific (local) interpretabilities. Experimental evaluation demonstrate that our in-database probabilistic approach provides the same interpretability quality as the precise space-inefficient approach, while providing scalable and space efficient runtime behavior (up to 8X space savings), without any user intervention.

==> aidb.tex <==
\section{AI-Powered Database}
\label{sec:aidb}
\vspace{0.2in}

\begin{figure}[htbp]
  \centering
  \includegraphics[width=\linewidth]{figures/aidbfig.pdf}
  \caption{Overview of the AI-Powered Database (AI-DB)}
  \label{fig:poverview}
\end{figure}

Figure \ref{fig:poverview} presents the three key phases in the execution flow of 
of an AI-Powered Database. The first training phase takes place when the
database is used to train the model (this phase is not needed when a pre-trained model is used). Our training approach is
characterized by two unique aspects: (1) Using \emph{meaningful} unstructured text
representation of the structured relational data as input to the
training process and (2) Using the \emph{self-supervised} vector embedding
technique to generate meaning vectors from the input text
corpus. AI-DB uses a specialized vector embedding approach, called database embedding,  to address various subtletiles with the relational
data model (e.g., supporting primary keys). After training, every unique token from the input corpus is associated with a
vector of dimension $d$. 

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figures/example.pdf}
  \caption{Building a model from an input relational database table in AI-DB}
  \label{fig:example}
\end{figure}


Following training (or reading from a pre-trained model), the resultant vectors are stored to be used for
 inference (phase 2).  In the third phase, a query execution engine uses
various semantic functions that first fetch the trained vectors as
needed and then use them to implement semantic contextual computations
in various Cognitive Intelligence (CI) queries.  Each CI query uses the UDFs to measure semantic similarity
between a pair of tokens associated with the
input relational parameters. The core computational operation of a cognitive UDF is to calculate similarity
between a pair of tokens by computing the cosine distance
between the corresponding vectors (\emph{nearest neighbor computations}). 
The cosine distance value varies from 1.0 (very similar) to -1.0 (very dissimilar). 

%For two vectors $v_1$ and
%$v_2$, the cosine distance is computed as $cos(v_1 , v_2 ) =
%%cos(v_1,v_2)=\frac{v_1\cdot v_2}{\lVert {v_1} \rVert \lVert
%  {v_2} \rVert}$. 

Our current implementation supports four types of CI queries:
similarity queries, inductive reasoning, prediction, and
cognitive OLAP~\cite{DBLP:journals/corr/abs-1712-07199}. These queries can be executed over databases with
multiple datatypes: we currently support text, numeric, and image
data. The \emph{similarity} queries compare two relational
variables based on similarity or dissimilarity between the input
variables. The inductive reasoning queries exploit latent semantic information in the database
to reason from \emph{part} to \emph{whole}, or from \emph{particular}
to \emph{general}. We support  different types of inductive
reasoning queries: analogies, semantic clustering, and
odd-man-out. Predictive queries cover traditional classification as
well as semantic queries over unseen (untrained) data. Finally, cognitive OLAP allows SQL
aggregation functions such as \texttt{MAX()}, \texttt{MIN()} or
\texttt{AVG()} over a set that is identified by contextual similarity
computations on the relational variables. There are multiple ways of
implementing CI queries: as SQL queries with either User-defined or system built-in functions implemented in C/C++ or Scala, or as Python functions.

For the subsequent sections, we will use the following defitions for the terminology.  {\em Textification} of a relational table is defined as the conversion of a relational table view into text entries. All unique fields in a column
are converted into categorical strings. Numerical value is converted into strings by clustering and assigned categorical
values. A {\em token} is defined as an unique string value in a relational field (row, column location).  A {\em query} is defined as presenting
a query token to the AI DB, in order to find other tokens that are most closely related based on some criteria (embedding similarity, semantic or analogy). Queries may be restricted by columns or provided additional constraints.




==> background.tex <==
\section{Introduction}

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figures/aidbfig.pdf}
  \caption{AI-DB Methodology}
  \label{fig:poverview}
\end{figure}

AI-DB has been proposed in prior work to enable a closer connection between database systems and AI techniques. We will briefly review the AI-DB environment within which the interpretability solutions are proposed.

Figure \ref{fig:poverview} presents the three key phases in the execution flow of 
of an AI-Powered Database. The first training phase takes place when the
database is used to train the model (this phase is not needed when a pre-trained model is used). Our training approach is
characterized by two unique aspects: (1) Using \emph{meaningful} unstructured text
representation of the structured relational data as input to the
training process and (2) Using the \emph{self-supervised} vector embedding
technique to generate meaning vectors from the input text
corpus. We have modified the classical word embedding
approach~\cite{mikolov:corr-abs-1301-3781} to address various subtletiles with the relational
data model (e.g., supporting primary keys). After training, every unique token from the input corpus is associated with a
vector of dimension $d$. 

Following training (or reading from a pre-trained model), the resultant vectors are stored to be used for
 inference (phase 2).  In the third phase, a query execution engine uses
various user-defined functions (UDFs) that first fetch the trained vectors as
needed and then use them to implement semantic contextual computations
in various Cognitive Intelligence (CI) queries.  Each CI query uses the UDFs to measure semantic similarity
between a pair of sets (or sequences) of tokens associated with the
input relational parameters. The core computational operation of a cognitive UDF is to calculate similarity
between a pair of tokens by computing the cosine distance
between the corresponding vectors (\emph{nearest neighbor computations}). 
The cosine distance value varies from 1.0 (very similar) to -1.0 (very dissimilar). 

%For two vectors $v_1$ and
%$v_2$, the cosine distance is computed as $cos(v_1 , v_2 ) =
%%cos(v_1,v_2)=\frac{v_1\cdot v_2}{\lVert {v_1} \rVert \lVert
%  {v_2} \rVert}$. 

Our current implementation supports four types of CI queries:
similarity queries, inductive reasoning, prediction, and
cognitive OLAP~\cite{DBLP:journals/corr/abs-1712-07199}. These queries can be executed over databases with
multiple datatypes: we currently support text, numeric, and image
data. The \emph{similarity} queries compare two relational
variables based on similarity or dissimilarity between the input
variables. The inductive reasoning queries exploit latent semantic information in the database
to reason from \emph{part} to \emph{whole}, or from \emph{particular}
to \emph{general}. We support  different types of inductive
reasoning queries: analogies, semantic clustering, and
odd-man-out. Predictive queries cover traditional classification as
well as semantic queries over unseen (untrained) data. Finally, cognitive OLAP allows SQL
aggregation functions such as \texttt{MAX()}, \texttt{MIN()} or
\texttt{AVG()} over a set that is identified by contextual similarity
computations on the relational variables. There are multiple ways of
implementing CI queries: as SQL queries with UDFs implemented in C/C++
or Scala, or as Python functions.

For the subsequent sections, we will use the following defitions for the terminology.
{\em Textification} of a DB2 table is defined as the conversion of a DB2 Table view into text entries. All unique fields in a column
are converted into categorical strings. Numerical value is converted into strings by clustering and assigned categorical
values. A {\em token} is defined as an unique string value in a DB2 field (row, column location).  A {\em query} is defined as presenting
a query token to the AI DB, in order to find other tokens that are most closely related based on some criteria (embedding similarity, semantic or analogy). Queries may be restricted by columns or provided additional constraints.




==> sketch.tex <==
\section{Sparse Scalable Sketch}
\label{sec:sketch}
\vspace{0.3in}


Data sketches are probabilistic structures used for compression and
compactly recording tokens in streams for prespecified queries. Common
queries typically supported are total counts of tokens seen in a
stream or database, and a variety of algorithms such a Count-Min
sketch have been developed for this purpose.  Structurally, count-min
sketches~\cite{DBLP:journals/corr/PitelF15,journals/jal/CormodeM05,DBLP:journals/corr/abs-1902-10995}
are typically implemented as two-dimensional tables, each row indexed
by a different hash function.  During query, a count summarization
performed across the rows using a pre-specified algorithm such as a
minimum function.  The use of sketches for NLP in particular has been
presented in ~\cite{goyal-etal-2010-sketching}.  
 
In our design, count-Min sketches are updated with token pair
co-occurrence in a textified database used for cognitive AI.  The
table and the update process is shown in Figure~\ref{fig:occurupdate}.
Co-occurrence counts between column tokens of AI DB textified data
strings are tracked and incremented in the sketch. 

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figures/churn-sketch.pdf}
\caption{Sketch Count Updates}
\label{fig:occurupdate}
\end{figure}

The benefit of using large sketches for updates is that they can be
represented by sparse matrices as shown in
Figure~\ref{fig:sparsematrix}. The ability to increase the size of the
sketch while allowing the sparsity gives the best of both worlds:
accuracy in interpretability, while allowing for space and performance
afforded by sparse matrix techniques. 

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figures/sketchsparsematrix.pdf}
\caption{Sketch as Sparse Matrix}
\label{fig:sparsematrix}
\end{figure}


%\begin{figure}[h]
%\centering
%\includegraphics[angle=-90,width=\linewidth]{figures/shadowsketch.pdf}
%\caption{Sparse Sketch with Shadow}
%\label{fig:shadowsketch}
%\end{figure}


\begin{table}
\caption{Unique Co-occurring Token Pairs}
\centering
\begin{tabular}{ll}
\toprule
\multicolumn{1}{c}{Datasets} & \multicolumn{1}{c}{Unique} \\
 &  \multicolumn{1}{c}{Token Pairs}   \\ 
\cmidrule(lr){2-2}
Telco Customer Churn               & 1527        \\ 
Fannie Mae                         & 202499        \\ 
Virginia                           & 1067565        \\ 
Credit Card Fraud                  & 10271049       \\ 
CA Toxicity                        & 13320509      \\ 
AML                                & 218388786       \\ 
\bottomrule
\end{tabular}
\label{table:uniquepairs}
\end{table}


For the purpose of interpretability of DB2 textified data, counts of
entries in columns need to be tracked, and well as their
co-occurrences.  In textified databases, particularly with large
numbers of unique values in the columns, the number of co-occurring
tokens can be high as shown in
Table~\ref{table:uniquepairs}. Alternatives to our solution with
sketches such as dictionaries in memory, with full strings as keys, is
prohibitive. Sketches provide compact and compressed, although
slightly approximate, structures to record counts of co-occurring
tokens.  We investigated the use of {\em sparse sketches} for compact
representations of SQLDB textified database co-occurrences as well as
counts of individual tokens.  Each row in the hash table is made
reasonably wide and deep, along with a CountMin algorithm,  so as to
minimize the impact of hash conflicts across the co-occuring
tokens. This results in a two-dimensional array that is quite sparse
and can be represented and operated on efficiently as a compact array
using sparse matrix representation techniques.  This enables the
representation of counts for a large number of co-occurrences in a
sparse memory-efficient manner. 

%\begin{figure}[h]
%\centering
%\includegraphics[width=\linewidth]{figures/sparsesketch.pdf}
%\caption{Sparse Sketch}
%\label{fig:poverview}
%\end{figure}


Each column in a DB2 table may have multiple possible values. In some
cases such as Customer Churn, the column may only have binary values
such as Yes/No, and in other cases such as Year, it could span tens or
hundreds of possible entries.  Consider two columns A and B, where A
has $m$ unique posible values and B has $n$ unique possible values.
The total number of co-occurring tokens the system may have to keep
track would be $mxn$.  Given k possible column, the total number of
co-occurences could be as high as $mxnxk$. 

\subsection{Shadow Containment Sketch}
\vspace{0.3in}
A common issue with sketches is that they are sufficiently accurate
when the number of tokens are limited, and queries are made within the
limited numbers of tokens.  If the universe of tokens that are used in
queries (such as tokens never seen before by the sketch) is much
larger than the sketch was designed for, the queries will produce
inaccurate counts.  This is common in database tables which have
columns with a large number of possible entries (such as account
numbers), and the totalk possible combinations, say in a database
transaction tracking to and from accounts, each with m and n possible
values would result in a large universe of mxn number of possible
co-occurring tokens; although the actual number of co-occurrences in
the database itself may be much smaller. Building sketches which store
counts for the large universe of all possible token co-ocurrences is
prohibitive in terms of memory. In order to address this, we only
query the count sketch for tokens that exist in the database, by using
a shadow boolean sketch that tracks which co-occurrences actually
exist in the database as opposed to all possible permutations of
co-occurrences that could occurr. Figures~\ref{fig:update} and
~\ref{fig:query} show the update and query of the sketch
respectively. 



\begin{figure}[h]
\centering
\includegraphics[angle=-90,width=\linewidth]{figures/query.pdf}
\caption{Sparse Sketch with Shadow Query}
\label{fig:query}
\end{figure}


\begin{figure}[h]
\centering
\includegraphics[angle=-90,width=\linewidth]{figures/update.pdf}
\caption{Sparse Sketch with Shadow Update}
\label{fig:update}
\end{figure}

A shadow sketch is a Bloom sketch, where each entry in the hashed rows
are boolean binary values. Since the shadow containment sketch only
records whether a token exists or does not exist in the count sketch,
a single bit may be used.  To improve the accuracy, deep sketches with
rows, each having different hashes are used. During a query each of
the rows are updated based on the hash function for that row. During a
query all rows are queried  and a boolean AND is performed across the
rows. 

\subsection{Thresholding to improve sparsity}
\vspace{0.3in}

The compression of the sketch can further be improved although at a
small impact on accuracy by {\em thresholding} small values in the
sketch and setting them to zero.  This makes the matrix sparser.
During interpretability, the sketch values are to be trusted for large
counts, for smaller counts the results are removed and or annotated
for the user by presenting discriminatory scores to show their small
counts. 


 When interpretability queries can be structured in a manner that only
 heavy hitters are presented in sorted order, then low frequency
 counts become less imnportant. In some cases, the low frequency
 counts can be removed altogether without a significant impact on the
 accuracy of the interpretability queries.  We determine low frequency
 in terms the median values of the frequencies of the co-occurring
 tokens. The median values among all co-occurring pairs are first
 computed, then a threshold is selected (as a fixed fraction of the
 median value). 

\subsection{Multiprocessing for Runtime Speedup}
\vspace{0.3in}
Approaches in previous sections focused on memory and space
improvements through the use of sketches. Runtime is another major
challenge facing the creation of sketches, especially as the size in
terms of the number of rows grows. The sketch creation algorithm has
to track the co-occurrence in every row, and therefore the runtime
grows linearly with the size of the text file. Sketches are inherently
distributive in nature. As long as the size of the sketch, and the
hash functions for each other rows are the same, i.e., the sketches
are compatible, they can be simply added together without loss of
accuracy. Speedup in processing can be achieved through
multiprocessing.  Each text file, can be split by rows into several
non-overlapping chunks, and separate count sketches are generated for
each chunk in parallel by separate threads.  Once the sketch
generation for the chunks is complete, the sketches generated by each
thread are merged together by adding the entries in the sketches into
a single top level sketch. 


